Quality-aware semi-supervised learning for CMR segmentation

One of the challenges in developing deep learning algorithms for medical image segmentation is the scarcity of annotated training data. To overcome this limitation, data augmentation and semi-supervised learning (SSL) methods have been developed. However, these methods have limited effectiveness as they either exploit the existing data set only (data augmentation) or risk negative impact by adding poor training examples (SSL). Segmentations are rarely the final product of medical image analysis - they are typically used in downstream tasks to infer higher-order patterns to evaluate diseases. Clinicians take into account a wealth of prior knowledge on biophysics and physiology when evaluating image analysis results. We have used these clinical assessments in previous works to create robust quality-control (QC) classifiers for automated cardiac magnetic resonance (CMR) analysis. In this paper, we propose a novel scheme that uses QC of the downstream task to identify high quality outputs of CMR segmentation networks, that are subsequently utilised for further network training. In essence, this provides quality-aware augmentation of training data in a variant of SSL for segmentation networks (semiQCSeg). We evaluate our approach in two CMR segmentation tasks (aortic and short axis cardiac volume segmentation) using UK Biobank data and two commonly used network architectures (U-net and a Fully Convolutional Network) and compare against supervised and SSL strategies. We show that semiQCSeg improves training of the segmentation networks. It decreases the need for labelled data, while outperforming the other methods in terms of Dice and clinical metrics. SemiQCSeg can be an efficient approach for training segmentation networks for medical image data when labelled datasets are scarce.

==> MICCAI_BR_2020 (1)/test.tex <==
%In the domain of computer vision, several works have proposed semi-supervised learning techniques, where labelled training data is augmented by data with image-level annotations, bounding boxes or scribbles \cite{lin2016cvpr,papandreou2015iccv}. 
\textcolor{red}{Alternatively, semi-supervised learning (SSL) methods have bee proposed to take advantage of unlabelled data during training. The most commonly used techniques for SSL include consistency training \cite{Rasmus2015}, pseudo labeling \cite{Lee2013}, entropy minimization \cite{Grandvalet2005}, bootstrapping \cite{Qiaoet2018} and generative modeling \cite{Hung2018}. However, most of these methods are designed for classification tasks, and its application in segmentation is still limited. Most common approaches focus on weakly-supervised learning \cite{Qiaoet2018, Radosavovic2018}, which consists of generating pseudo pixel-level labels to increase the training database and then train a segmentation network in a supervised manner. Another approach is to extend the generic GAN framework \cite{Hung2018} to pixel-level predictions, in this case the discriminator is then jointly trained with an adversarial loss and a supervised loss over the labeled examples. However, previous approaches has some limitation, for example in weakly-supervised approaches the segmentation network is trained with weakly labeled examples and hence they do not exploit the unlabeled data to extract additional training signal. While, methods based on adversarial training exploit the unlabeled data, but can be harder to train. For a review of semi-supervised learning techniques that have been proposed to take advantage of unlabelled data during training, see \cite{Cheplygina2019}}
In the medical imaging domain, Bai \textit{et al.,} proposed a semi-supervised learning approach for \textcolor{red}{CMR} image segmentation that combines labelled and unlabelled data during training \cite{Bai2017semisup}. \textcolor{red]{This technique uses a processing step before using new training samples, by applying a conditional random field algorithm (CRF) to smoothen the obtained segmentations.}. More recently, Kervadec \textit{et al.,} proposes a semi supervised algorithm for 3D left atrium segmentation. They use a teacher-student weakly supervise approach where the student model learns from the teacher model by minimizing the segmentation loss on the labeled data the consistency loss with respect to the targets from the teacher model on all input data.} \\
The benefits of standard data augmentation are limited by the variation present in the existing data, while neural network generated augmented samples and semi-supervised learning potentially suffer from generation of unrealistic or inaccurate examples. These are not insignificant drawbacks, particularly in medical image analysis. 
Our proposed method utilises aspects of data augmentation and semi-supervised learning alongside robust QC. It creates an approach for semi-supervised DL model training that is informed by an independent QC network, trained
using prior knowledge of biophysical behaviour in a downstream task. To the best of our knowledge, no previous authors have used such a QC-informed approach in semi-supervised image segmentation.



==> test.tex <==
%In the domain of computer vision, several works have proposed semi-supervised learning techniques, where labelled training data is augmented by data with image-level annotations, bounding boxes or scribbles \cite{lin2016cvpr,papandreou2015iccv}. 
\textcolor{red}{Alternatively, semi-supervised learning (SSL) methods have bee proposed to take advantage of unlabelled data during training. The most commonly used techniques for SSL include consistency training \cite{Rasmus2015}, pseudo labeling \cite{Lee2013}, entropy minimization \cite{Grandvalet2005}, bootstrapping \cite{Qiaoet2018} and generative modeling \cite{Hung2018}. However, most of these methods are designed for classification tasks, and its application in segmentation is still limited. Most common approaches focus on weakly-supervised learning \cite{Qiaoet2018, Radosavovic2018}, which consists of generating pseudo pixel-level labels to increase the training database and then train a segmentation network in a supervised manner. Another approach is to extend the generic GAN framework \cite{Hung2018} to pixel-level predictions, in this case the discriminator is then jointly trained with an adversarial loss and a supervised loss over the labeled examples. However, previous approaches has some limitation, for example in weakly-supervised approaches the segmentation network is trained with weakly labeled examples and hence they do not exploit the unlabeled data to extract additional training signal. While, methods based on adversarial training exploit the unlabeled data, but can be harder to train. For a review of semi-supervised learning techniques that have been proposed to take advantage of unlabelled data during training, see \cite{Cheplygina2019}}
In the medical imaging domain, Bai \textit{et al.,} proposed a semi-supervised learning approach for \textcolor{red}{CMR} image segmentation that combines labelled and unlabelled data during training \cite{Bai2017semisup}. \textcolor{red]{This technique uses a processing step before using new training samples, by applying a conditional random field algorithm (CRF) to smoothen the obtained segmentations.}. More recently, Kervadec \textit{et al.,} proposes a semi supervised algorithm for 3D left atrium segmentation. They use a teacher-student weakly supervise approach where the student model learns from the teacher model by minimizing the segmentation loss on the labeled data the consistency loss with respect to the targets from the teacher model on all input data.} \\
The benefits of standard data augmentation are limited by the variation present in the existing data, while neural network generated augmented samples and semi-supervised learning potentially suffer from generation of unrealistic or inaccurate examples. These are not insignificant drawbacks, particularly in medical image analysis. 
Our proposed method utilises aspects of data augmentation and semi-supervised learning alongside robust QC. It creates an approach for semi-supervised DL model training that is informed by an independent QC network, trained
using prior knowledge of biophysical behaviour in a downstream task. To the best of our knowledge, no previous authors have used such a QC-informed approach in semi-supervised image segmentation.


